Discriminative Ordering Through Ensemble Consensus

Evaluating the performance of clustering models is a challenging task where the outcome depends on the definition of what constitutes a cluster. Due to this design, current existing metrics rarely handle multiple clustering models with diverse cluster definitions, nor do they comply with the integration of constraints when available. In this work, we take inspiration from consensus clustering and assume that a set of clustering models is able to uncover hidden structures in the data. We propose to construct a discriminative ordering through ensemble clustering based on the distance between the connectivity of a clustering model and the consensus matrix. We first validate the proposed method with synthetic scenarios, highlighting that the proposed score ranks the models that best match the consensus first. We then show that this simple ranking score significantly outperforms other scoring methods when comparing sets of different clustering algorithms that are not restricted to a fixed number of clusters and is compatible with clustering constraints.

==> figures/table_benchmark_correlation_gain.tex <==
\begin{table*}[t]
	\centering
	\caption{Kendall's tau correlation ($\uparrow$) before ($\emptyset$) and after adding regularisation ($\mathcal{R}$) using must-link cannot-link constraints from 20 random nodes for the UCI datasets.}
	\label{tab:benchmark_correlation_gain}
	\begin{tabular}{lrlrlrlrl}
		\toprule
		Dataset  & \multicolumn{2}{c}{AARI} & \multicolumn{2}{c}{ANMI} & \multicolumn{2}{c}{KL} & \multicolumn{2}{c}{Binary}\\
		& $\emptyset$ & $\mathcal{R}$ &  $\emptyset$ & $\mathcal{R}$ &  $\emptyset$ & $\mathcal{R}$ &  $\emptyset$ & $\mathcal{R}$ \\
		\midrule
		Dermatology & 0.49 & 0.77\std{0.06} & 0.73 & \textbf{0.79\std{0.05}} & 0.58 & 0.76\std{0.04} & 0.41 & 0.75\std{0.05} \\
		Digits & -0.21 & 0.73\std{0.06} & 0.40 & 0.76\std{0.06} & -0.47 & 0.78\std{0.05} & 0.73 &\textbf{0.84\std{0.04}} \\
		Glass & \textbf{0.70} & 0.39\std{0.11} & 0.40 & 0.29\std{0.07} & \textbf{0.70} & 0.45\std{0.11} & 0.69 & 0.64\std{0.11} \\
		Ionosphere & 0.23 & 0.68\std{0.11} & -0.04 & 0.56\std{0.15} & 0.36 & 0.72\std{0.10} & 0.48 & \textbf{0.74\std{0.09}} \\
		Iris & 0.66 & 0.63\std{0.09} & 0.37 & 0.38\std{0.20} & 0.05 & 0.27\std{0.21} & 0.69 & \textbf{0.72\std{0.03}} \\
		Lung & 0.27 & 0.34\std{0.04} & 0.14 & 0.16\std{0.03} & 0.18 & 0.21\std{0.03} & 0.27 & \textbf{0.43\std{0.05}} \\
		Segmentation & 0.48 & \textbf{0.77\std{0.06}} & 0.49 & 0.75\std{0.04} & 0.35 & 0.71\std{0.10} & 0.39 & 0.64\std{0.10} \\
		Wdbc & 0.02 & 0.35\std{0.17} & 0.40 &\textbf{0.57\std{0.18}} & 0.29 & 0.43\std{0.14} & 0.54 & \textbf{0.57\std{0.15}} \\
		Wine & 0.27 & 0.70\std{0.05} & 0.40 & 0.64\std{0.04} & 0.77 & 0.75\std{0.03} & \textbf{0.79} & \textbf{0.79\std{0.03}} \\
		\bottomrule
	\end{tabular}
\end{table*}

==> figures/table_benchmark_fixed_regretkendall_restricted.tex <==
\begin{table}[t]
    \centering
    \caption{Regret on the Kendall tau correlation\std{std} ($\downarrow$) of the ranking metrics when the base clusterings are restricted to as many clusters as targets. KL and Binary respectively stand for the DISCOTEC with KL divergence, and consensus binarisation.}
    \label{tab:benchmark_fixed_regretkendall_restricted}
    \begin{tabular}{lllll}
        \toprule
        &\multicolumn{2}{c}{FCPS}&\multicolumn{2}{c}{UCI}\\
        \cmidrule(r){2-3}\cmidrule(l){4-5}
        Model & Agg. & Kmeans & Agg. & Kmeans \\
        \midrule
        AARI & 0.40\std{0.48} & 0.78\std{0.84} &1.31\std{0.65} & 0.62\std{0.50} \\
        ANMI & 0.30\std{0.48} & 0.81\std{0.82} &1.28\std{0.59} & 0.57\std{0.54} \\
        CHI & 0.52\std{0.49} & 0.34\std{0.46} &\textbf{0.01\std{0.03}} & 0.69\std{0.53} \\
        SI & 0.81\std{0.73} & \textbf{0.16\std{0.23}} &1.42\std{0.45} & 0.42\std{0.47} \\
        \cmidrule{2-5}
        KL & 0.50\std{0.68} & 0.79\std{0.83} &1.49\std{0.52} & 0.62\std{0.50} \\
        Binary & \textbf{0.15\std{0.21}} & 0.82\std{0.96} &0.52\std{0.65} & 0.62\std{0.50} \\
        \bottomrule
    \end{tabular}
\end{table}

==> figures/table_benchmark_mixed_regretkendall_restricted.tex <==
\begin{table*}[t]
    \centering
    \caption{Regret on the Kendall tau correlation\std{std} ($\downarrow$) of the ranking metrics when the base clusterings seek different number of clusters.}
    \label{tab:benchmark_mixed_regretkendall_restricted}
    \begin{tabular}{lllllllll}
        \toprule
        &\multicolumn{4}{c}{FCPS}&\multicolumn{4}{c}{UCI}\\
        \cmidrule(r){2-5}\cmidrule(l){6-9}
        Model & Agg. & DBSCAN & Kmeans & Alltogether& Agg. & DBSCAN & Kmeans & Alltogether \\
        \midrule
        AARI & 0.47\std{0.32} & 0.26\std{0.34} & 0.65\std{0.35} & 0.55\std{0.39} &0.55\std{0.40} & 0.64\std{0.55} & 0.46\std{0.36} & 0.31\std{0.30} \\
        ANMI & 0.64\std{0.42} & 0.25\std{0.36} & 0.83\std{0.46} & 0.69\std{0.48} &0.43\std{0.40} & 0.67\std{0.54} & 0.65\std{0.45} & 0.26\std{0.13} \\
        CHI & 0.80\std{0.35} & 0.55\std{0.74} & 0.71\std{0.47} & 0.86\std{0.51} &0.35\std{0.25} & 0.44\std{0.34} & 0.31\std{0.42} & 0.26\std{0.26} \\
        SI & 0.74\std{0.31} & 0.72\std{0.63} & 0.54\std{0.35} & 0.81\std{0.44} &1.04\std{0.42} & 1.01\std{0.69} & 0.40\std{0.28} & 0.74\std{0.22} \\
        \cmidrule{2-9}
        KL & 0.56\std{0.48} & 0.31\std{0.44} & 1.01\std{0.48} & 0.62\std{0.51} &0.67\std{0.48} & 0.66\std{0.51} & 0.74\std{0.52} & 0.31\std{0.38} \\
        Binary & \textbf{0.02\std{0.07}} & \textbf{0.05\std{0.14}} & \textbf{0.03\std{0.05}} & \textbf{0.09\std{0.25}} &\textbf{0.10\std{0.20}} & 0.29\std{0.31} & \textbf{0.17\std{0.29}} & \textbf{0.11\std{0.13}} \\
        \bottomrule
    \end{tabular}
\end{table*}

==> figures/table_distance_cases.tex <==
\begin{table}[th]
    \centering
    \caption{Possible combinations of Bernoulli parameters and their simplifications  when computing the distance between a connectivity matrix and a consensus matrix.}
    \label{tab:distance_cases}
    \begin{tabular}{r c c}
        \toprule
        &$\pmb{A}^t_{ij}=0$&$\pmb{A}^t_{ij}=1$\\
        \midrule
        $\pmb{C}_{ij}=0$&0&Impossible\\
        $\pmb{C}_{ij} \in ]0,1[$&$D(\mathcal{B}(0) \| \mathcal{B}(\pmb{C}_{ij}))$&$D(\mathcal{B}(1) \| \mathcal{B}(\pmb{C}_{ij}))$\\
        $\pmb{C}_{ij}=1$&Impossible&0\\
        \bottomrule
    \end{tabular}
\end{table}
